R2F: A Remote Retraining Framework for AIoT Processors with Computing Errors

AIoT processors fabricated with newer technology nodes suffer rising soft errors due to the shrinking transistor sizes and lower power supply. Soft errors on the AIoT processors particularly the deep learning accelerators (DLAs) with massive computing may cause substantial computing errors. These computing errors are difficult to be captured by the conventional training on general purposed processors like CPUs and GPUs in a server. Applying the offline trained neural network models to the edge accelerators with errors directly may lead to considerable prediction accuracy loss. To address the problem, we propose a remote retraining framework (R2F) for remote AIoT processors with computing errors. It takes the remote AIoT processor with soft errors in the training loop such that the on-site computing errors can be learned with the application data on the server and the retrained models can be resilient to the soft errors. Meanwhile, we propose an optimized partial TMR strategy to enhance the retraining. According to our experiments, R2F enables elastic design trade-offs between the model accuracy and the performance penalty. The top-5 model accuracy can be improved by 1.93%-13.73% with 0%-200% performance penalty at high fault error rate. In addition, we notice that the retraining requires massive data transmission and even dominates the training time, and propose a sparse increment compression approach for the data transmission optimization, which reduces the retraining time by 38%-88% on average with negligible accuracy loss over a straightforward remote retraining.

==> diff.tex <==
\section{Difference List}
The difference between the manuscript and the conference version is listed as follows.

\begin{itemize}
\item We improve the on-site training to support remote AIoT processors and has the retraining built on top of Thingsboard, a representative IoT software stack, while the conference version mainly investigates the retraining of the faulty neural network accelerators on FPGAs.

\item We observe that the intermediate data transmission required by the retraining from AIoT processor to the server is time-consuming and even dominates the retraining under the IoT scenario with limited communication bandwidth, which is rather different from the retraining on the system in which the GPUs and deep learning accelerator are close to each other. To address the new problem, we take advantage of TMR to approximate the reference data and propose a sparse increment compression approach based on the approximated reference data. With this approach, we only need to transmit the compressed increments rather than the original outputs, which can greatly reduce the data transmission overhead and the retraining time accordingly.

\item We replace the original old neural networks with popular lightweight neural networks as the benchmark, including ResNet18, ResNet50, SqueezeNet, MobileNet and ShuffleNet, to represent typical AIoT applications. The old neural networks like VGG have more parameter redundancy and leave more space for retraining, which may affect the fault-tolerance analysis. In contrast, the lightweight neural network has less redundancy, the analysis is more practical.

\item We also intensively exploit the use of partial TMR on top of the proposed retraining framework and discuss the design trade-offs between the accuracy improvement and the performance penalty, which may shed light on designers with distinct requirements. While the conference paper has only one layer protected and assume that the protected layer is completely fault-free, this approach cannot be effectively applied for the lightweight neural network models and fails to scale under different fault error rates and application requirements.  

\item We also reorganize the paper and focus on resilient deep learning on AIoT processors rather than FPGA-based on-site retraining.

\end{itemize}

\section{\textcolor{red}{Replies to the reviewers}}
Thank you very much for all the insightful reviews and suggestions.

\vspace{1em}
For Reviewer 1:

\textbf{Q1: The soft error model in this work is not clear and may need better elaboration. Is the deployed model the good one or the bad one that have already been impacted by the soft errors?} Soft errors are randomly distributed to all the memory cells of the neural network accelerator including the register file and the on-chip buffer. When a memory cell is affected by soft errors, the data in the memory cell will be flipped. The soft error rate i.e., bit error rate is defined as the ratio of the bit faults over the total number of the memory cells. As the soft errors in the register file and input/output/weight buffers essentially affect the input and output of each MAC (multiply-accumulate), we have the influence of the soft errors in the neural network accelerator converted to the random bit flip of both the input and output of each basic MAC in the neural network processing. This approach makes it convenient to analyze the fault-tolerance of the neural network processing without low-level logic simulation. It has been adopted in prior fault analysis works as well [1-8] and the authors in [14] further demonstrated the potential fault analysis accuracy with more fine-grained consideration. The major problem is that it can only evaluates faults in algorithm-level and ignores the faults in controlling logic of the accelerator.

The model deployed in the experiment is the good one, but the computation of the model including the input, hidden states and output is impacted by the soft errors. We also elaborate the soft error model in Fault Injection Paragraph in Section VI-A according to this suggestion.


\textbf{Q2: It is not clear how to evaluate the accuracy with retraining under different BER assumption, in Figure 2. What specific fault-tolerant neural network processing techniques do you use? Specifically, how do you retrain to recover the accuracy of the target model? By introducing in-situ faults of adding regularization or penalty terms, or adding constraints?} We perform retraining for each different BER setup. This is also one of the motivations that we emphasize the in-situ retraining as shown in Section III. It is true that there are already some fault-tolerant training approaches like adding regularization, penalty terms and adding constraints as summarized in Section IV-A-2 in Page 11 in [15]. These approaches essentially add specialized constraints to the loss calculation. Nevertheless, they belong only one of the three different ways of fault-tolerant training. The in-situ fault tolerant training used in this paper does not modify the loss calculation and it has faults injected to the forward propagation such that the influence of the faults is reflected directly in the loss used in the backward propagation. As shown in Equation (1-4), the loss is essentially a statistic metric that averages the model induced errors as well as the various fault-induced computing errors. Basically, the training already takes the different faults into consideration. The resulting model can be tolerant to all the different faults rather than only the weight faults as demonstrated in the experiments. In addition, the training strategy is generally the same with that used in methods like disturbance/noise training in theory, which does not need to modify the loss function. The major difference is that the in-situ training needs to obtain the exact errors via in-situ calculation. Last but not least, the proposed data transmission optimizations can be applied to any in-situ training despite the different loss calculation approaches, because the data transmission turns out to be the bottleneck rather the model computation given limited AIoT uplink bandwidth. 

The mathematical formulation of the convolutional layer can be represented as:
\begin{equation}
\label{eq:conv}
    X^{i}=f(W^{i}\otimes  X^{i-1}+b^{i}) \qquad {\forall} i\in [1,L]
\end{equation}

Where $L$ is the number of layers in the network, while $f()$ is the non-linear activation function, e.g., a rectified linear unit (ReLU). Specifically, $X^{0}$ is the input images and $X^{L}$  is the output of the network. The loss can be formulated as:
\begin{equation}
\label{eq:loss}
\underset{\{{{W}^{i}}\}_{i=1}^{L}}{\mathop{\min }}\,Loss\left( {{X}^{0}},\{{{W}^{i}}\}_{i=1}^{L},label \right)
\end{equation}

When the faults are injected, the convolution calculation is as follows:
\begin{equation}
\label{eq:fault-conv}
X^{i}=f((W^{i}+{E_{W^{i}}}) \otimes (X^{i-1}+{E_{X^{i}}})+b^{i})
\end{equation}

where $E$ is the noise caused by faults injection and it is dynamic or random because of the characteristic of the in-situ faults in the accelerator. The loss with the fault injection can be formulated as below:
\begin{equation}
\label{eq:fault-loss}
\underset{\{{{W}^{i}}\}_{i=1}^{L}}{\mathop{\min }}\,Loss\left( {{X}^{0}},\{{{W}^{i}}\}_{i=1}^{L},\{{E_{W^{i}}}\}_{i}^{L},\{{E_{W^{i}}}\}_{i}^{L},label \right)
\end{equation}

By comparing Equation (2) and (4), we notice that the fault induced errors are already considered in the loss though the loss function is not changed.

\textbf{Q3: The soft error impacts the weights, inputs, and outputs as well as the hidden states of neural networks. Retraining only works for the weights part right? For the soft errors in input or output, why retraining can recover the accuracy?} As discussed in answer to Q2, although the in-situ retraining only changes the weights, it does not mean that the resulting model can only tolerate the weight faults. Because the loss already takes the various fault-induced errors considered in loss calculation according to Equation (4). Meanwhile, our experiments have the various faults including input faults, output faults and hidden state faults injected and the retrained models show improved model precision, which also demonstrates that the retraining can be used to tolerate the different faults other than the weight faults.


\textbf{Q4: To me, the reason why it is necessary to retrain in the AIoT is not clear. Why the BER cannot been modeled?} It is possible to measure the soft error rate of a specific chip and environment, [16] surveys the possible measurements. However, soft error rate measuring is challenging from the following aspects. First, the major soft error measuring methods including the accelerated SER (soft error rate) and the ‘real-time’ SER [16] requires specialized apparatus like radiation injector or ATE (automatic test equipment), which not only costs but also implicates many strict assumptions. For instance, it assumes that the chip working environments to be used are known in advance and remain unchanged. Also, the soft error rate is the same across the different chips and does not change with time. These assumptions are limited. Second, soft error rate can be dramatically affected by device-specific issues like process variation [17]. Hence, the soft errors can be non-uniform across the chip. The error distribution is also critical to characterize the soft errors, but it is usually expensive to measure and model the soft error distribution in practice. In addition, the device-specific soft error characteristic further complicates the measurement. In contrast, in-situ training avoids the imprecise and expensive measurements, which is more attractive for fault-tolerant neural network processing.


\textbf{Q5: Could you show more evidence that soft error would be an important issue for the accuracy degradation in AIoTs. As claimed in this work “the prediction accuracy of the neural network models drops little when BER is lower than $5\times 10^{-6}$”. what is the typical BER for the industrial AIoTs (let us assume it is fabricated with 7nm)?} This is a very good question and we are aware of the importance of the soft error rate metric as well. However, there is still a lack of references that clearly characterize the soft error rate under specific environments such as aerospace, radiation environment and automotive vehicle. To that end, we investigate the soft error rate utilized in related works. As shown in the Table \ref{SEU}, it can be seen that there are generally two different types of soft error metrics. One of them characterizes the soft errors from the perspective of the applications and it converts the soft error rate to bit flip probability of an operation or a memory cell. In this case, the fault analysis can be performed conveniently during the application execution on general purposed processors. The soft error rate used in [1-8] belongs to this category. The other type of soft error rate metric utilizes FIT/Mb, which is oriented to the real hardware [9-13]. However, the former metric usually implicates harsh environments while the latter metric typically targets specific semiconductor under normal working environments. Currently, we adopt the first category of the soft error metric, because our work mainly investigates when and how the fault-tolerant retraining can be beneficial rather than training for a specific safety-critical application. In fact, our experiments reveal that the in-situ retraining has its own applicable scope, which is probably related with the model fault tolerance limit. When the soft error rate is low, the errors can be tolerated without any modification. When the soft error rate is extremely high, dramatic accuracy drop is inevitable under even fully TMR protection. In this case, micro-architecture level or circuit level fault-tolerant approaches are required.
\begin{table}
    \centering
  \caption{The error rate for different error type}
  \label{SEU}
  \begin{tabular}{ccc}
    \toprule  
      Reference & Error Type & Error Rate \\
    \midrule
      $[1]$ & SEU & $1 \times 10^{-9}$ $\sim$ $1 \times 10^{-1}$ bit error rate  \\
      $[2]$ & SEU & $3 \times 10^{-6}$ $\sim$ $1 \times 10^{-4}$ per MAC  \\
      $[3]$ & SEU & $1$\% $\sim$ $10$\% per MAC  \\
      $[4]$ & SEU & $1 \times 10^{-5}$ $\sim$ $1 \times 10^{-1}$ bit error rate  \\
      $[5]$ & SEU & $1 \times 10^{-6}$ $\sim$ $1 \times 10^{-2}$ bit error rate  \\
      $[6]$ & SEU & $1 \times 10^{-5}$ $\sim$ $1 \times 10^{-1}$ bit error rate  \\
      $[7]$ & SEU & $1 \times 10^{-6}$ $\sim$ $1 \times 10^{-2}$ bit error rate  \\
      $[8]$ & SEU & $1 \times 10^{-8}$ $\sim$ $1 \times 10^{-4}$ bit error rate  \\
      $[9]$ & SEU (SRAM) & $157.62$ FIT/Mb, Vdd=$1$V, $28$nm \\
      $[10]$ & SEU (SRAM) & $741$ FIT/Mb, Vdd=$0.5$V, $28$nm \\
      $[11]$ & SEU (D-FF) & $0.18$ FIT/MFF, Vdd=$0.55$V, $7$nm \\
      $[12]$ & SEU (SRAM) & $80000$ FIT/Mb, Vdd=$0.22$V, $7$nm FinFET \\
      $[13]$ & SEU & $0.39$ FIT/Mb \\
  \bottomrule
\end{tabular}
\vspace{-1em}
\end{table}

In addition, we argue that soft errors are of vital importance from the perspective of many safety-critical AIoT applications. For example, many smart cameras used in automotive vehicles, ADAS systems, and unmanned aerial vehicles greatly rely on robust neural network processing to avoid collision or other obstacles to ensure safety. Wrong prediction caused by the soft errors will increase the probability of the system failures and even lead to catastrophic consequences. Robots for dangerous tasks like radioactive waste disposal can suffer severe soft errors caused by the radiation, and the embedded intelligent processors must be protected against the soft errors.

\vspace{3em}

\noindent
[1] Reagen, Brandon, Udit Gupta, Lillian Pentecost, Paul Whatmough, Sae Kyu Lee, Niamh Mulholland, David Brooks, and Gu-Yeon Wei. "Ares: A framework for quantifying the resilience of deep neural networks." In 2018 55th ACM/ESDA/IEEE Design Automation Conference (DAC), pp. 1-6. IEEE, 2018.

\noindent
[2] Ning, Xuefei, Guangjun Ge, Wenshuo Li, Zhenhua Zhu, Yin Zheng, Xiaoming Chen, Zhen Gao, Yu Wang, and Huazhong Yang. "FTT-NAS: Discovering Fault-Tolerant Neural Architecture." arXiv preprint arXiv:2003.10375 (2020).

\noindent
[3] Li, Wenshuo, Xuefei Ning, Guangjun Ge, Xiaoming Chen, Yu Wang, and Huazhong Yang. "FTT-NAS: discovering fault-tolerant neural architecture." In 2020 25th Asia and South Pacific Design Automation Conference (ASP-DAC), pp. 211-216. IEEE, 2020.

\noindent
[4] Li, Wenshuo, Guangjun Ge, Kaiyuan Guo, Xiaoming Chen, Qi Wei, Zhen Gao, Yu Wang, and Huazhong Yang. "Soft Error Mitigation for Deep Convolution Neural Network on FPGA Accelerators." In 2020 2nd IEEE International Conference on Artificial Intelligence Circuits and Systems (AICAS), pp. 1-5. IEEE, 2020.

\noindent
[5] Ozen, Elbruz, and Alex Orailoglu. "Sanity-Check: Boosting the reliability of safety-critical deep neural network applications." In 2019 IEEE 28th Asian Test Symposium (ATS), pp. 7-75. IEEE, 2019.

\noindent
[6] Banerjee, Subho S., James Cyriac, Saurabh Jha, Zbigniew T. Kalbarczyk, and Ravishankar K. Iyer. "Towards a Bayesian Approach for Assessing Fault Tolerance of Deep Neural Networks." In 2019 49th Annual IEEE/IFIP International Conference on Dependable Systems and Networks–Supplemental Volume (DSN-S), pp. 25-26. IEEE, 2019.

\noindent
[7] Schorn, Christoph, Andre Guntoro, and Gerd Ascheid. "An efficient bit-flip resilience optimization method for deep neural networks." In 2019 Design, Automation \& Test in Europe Conference \& Exhibition (DATE), pp. 1507-1512. IEEE, 2019.

\noindent
[8] Mahdiani, Hamid Reza, Sied Mehdi Fakhraie, and Caro Lucas. "Relaxed fault-tolerant hardware implementation of neural networks in the presence of multiple transient errors." IEEE transactions on neural networks and learning systems 23, no. 8 (2012): 1215-1228.

\noindent
[9] Li, Guanpeng, Siva Kumar Sastry Hari, Michael Sullivan, Timothy Tsai, Karthik Pattabiraman, Joel Emer, and Stephen W. Keckler. "Understanding error propagation in deep learning neural network (DNN) accelerators and applications." In Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis, pp. 1-12. 2017.

\noindent
[10] Neale, Adam, and Manoj Sachdev. "Neutron radiation induced soft error rates for an adjacent-ECC protected SRAM in 28 nm CMOS." IEEE Transactions on Nuclear Science 63, no. 3 (2016): 1912-1917.

\noindent
[11] Cao, J., L. Xu, Bharat L. Bhuva, S-J. Wen, R. Wong, Balaji Narasimham, and Lloyd W. Massengill. "Alpha Particle Soft-Error Rates for D-FF Designs in 16-Nm and 7-Nm Bulk FinFET Technologies." In 2019 IEEE International Reliability Physics Symposium (IRPS), pp. 1-5. IEEE, 2019.

\noindent
[12] Narasimham, Balaji, Saket Gupta, Dan Reed, J. K. Wang, Nick Hendrickson, and Hasan Taufique. "Scaling trends and bias dependence of the soft error rate of 16 nm and 7 nm FinFET SRAMs." In 2018 IEEE International Reliability Physics Symposium (IRPS), pp. 4C-1. IEEE, 2018.

\noindent
[13] Luza, Lucas Matana, Daniel Söderström, Georgios Tsiligiannis, Helmut Puchner, Carlo Cazzaniga, Ernesto Sanchez, Alberto Bosio, and Luigi Dilillo. "Investigating the Impact of Radiation-Induced Soft Errors on the Reliability of Approximate Computing Systems." In 2020 IEEE International Symposium on Defect and Fault Tolerance in VLSI and Nanotechnology Systems (DFT), pp. 1-6. IEEE, 2020.

\noindent
[14] He, Yi, Prasanna Balaprakash, and Yanjing Li. "FIdelity: Efficient Resilience Analysis Framework for Deep Learning Accelerators." In 2020 53rd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO), pp. 270-281. IEEE, 2020.

\noindent
[15] Torres-Huitzil, Cesar, and Bernard Girau. "Fault and error tolerance in neural networks: A review." IEEE Access 5 (2017): 17322-17341.

\noindent
[16] Autran, Jean-Luc, Daniela Munteanu, Philippe Roche, and Gilles Gasiot. "Real-time soft-error rate measurements: A review." Microelectronics Reliability 54, no. 8 (2014): 1455-1476.

\noindent
[17] Qian Ding, Rong Luo and Yuan Xie, "Impact of process variation on soft error vulnerability for nanometer VLSI circuits," 2005 6th International Conference on ASIC, Shanghai, China, 2005, pp. 1117-1121.



\vspace{1em}
For Reviewer 2:

\textbf{Q1: If I understand correctly, the experiments are done for epoch=1 as mentioned at the end of section VI-A in page 7, right column. How the accuracy changes for different epoch values? Assuming accuracy increases in the “base” model for large epoch values even with soft-erros, is that closes the accuracy gap between the proposed method and “base” model?} Yes, the training had epoch set to 1 in the experiments. We take ResNet18 as an example and evaluated the model accuracy under different epoch setups according to your suggestion. Also we add this to the end of the experiment section. The experiment result is shown in Figure \ref{fig:epochinfluence}. It can be observed that the retrained model accuracy shows little improvement given larger epoch. The main reason is that the fault-tolerant retraining is based on top of a pretrained model rather than a totally new training. In this case, a single epoch is sufficient according to our experiments. If the model is trained from scratch, epoch needs to be much larger. 

\begin{figure}
\centering
    \includegraphics[width=0.45\textwidth]{figures/epochinfluence.pdf}
    \vspace{-0.5em}
    \caption{The influence of different epoch setups on the proposed R2F training.}
\label{fig:epochinfluence}
\vspace{-1em}
\end{figure}

\vspace{1em}
For Reviewer 3:

\textbf{Q1: The paper proposes a retraining framework for neural networks on IoT devices. My major concern is that the paper is more towards an implementation and engineering paper, but lacks the theoretical technical contribution from a research perspective. The fault-tolerant neural networks have been well studied in the existing literatures including [19],[21]. More importantly, the error/fault-aware retraining have been studied intensively as well, and some important references are missing. Thus, the paper has done a nice job in implementing the remote retraining in the IoT context and I can see the merit of this being a well-developed demonstration, but unfortunately it lacks sufficient research merits.} It is true that the in-situ retraining is indicated in some prior works, but the inference is usually conducted on the accelerator that is close to the host processor. Thereby, the communication bandwidth is typically large and the data transmission will not induce too much overhead. In addition, the retraining is usually considered to be a non-frequent operation, which also makes the training overhead less important. Nevertheless, the problem is quite different under the AIoT scenario. First, the communication bandwidth especially the uplink bandwidth is rather limited in many AIoT devices. As a result, the data transmission time can be many times larger compared to the computing time of the retraining. Second, a server is usually shared by a larger number of AIoT devices. Although the device-specific retraining for a specific AIoT processor is non-frequent, the retraining from the perspective of the server can be non-trivial. Basically, the AIoT scenario makes the neural network in-situ training unique and we need to revisit the retraining framework which we take it for granted before for practical employment. We mainly address the retraining problem from the perspective of system design rather than the algorithm design. For instance, the retraining framework needs to be distributed and combined with the existing AIoT software stacks. Data transmission becomes the performance bottleneck of the remote in-situ retraining, it needs to be optimized. Thereby, we argue the remote retraining targeting resilient IoT intelligence is a new and important research problem. To address the problem, we presented an initial yet systematic solution and it works well according to our experiments. For the missing related work, we also review the related work carefully and improved the related works as highlighted Section II.


\textbf{Q2: Section V-A. “Then, we calculate the increments of the intermediate outputs relative to the approximate reference outputs on the AIoT processor with soft errors.”
Although the use of increments instead of the intermediate outputs can result in compress and savings of communication bandwidth, considering the non-trivial amount of intermediate outputs, how much overhead is introduced in the increment calculation than regular different types of neural networks?} As the number of subtraction operations required by the increment calculation equals to the number of output features and it is much smaller compared to the number of MAC operations in convolution, the computing overhead of the subtraction is negligible. Take a single convolution layer as an example. Suppose the input channel is $I$, the feature width is $W$. the feature height is $H$, convolution kernel size is $K$, output channel is $O$. The number subtraction is $O\times H \times W$, while the number of MACs in the convolution layer is $I \times H \times W \times K \times K \times O$ and it is $I \times K \times K$ times larger. In addition, MAC is more complex than the subtraction. The overhead is small as expected and it is included in model Dec/compression in Figure 6 in Page 9. We highlight the description about this.

\textbf{Q3: Section V-A. “Since they are not significantly different, the incremental results include a large number of zeros and can be compressed efficiently.” The reviewer is also interested to know the relationship between the compress ratio and the (soft) error rate. Knowing those results in the middle can provide a lot of information in addition to presented end-to-end results like accuracy and energy saving.} We analyzed the data compression rate and the soft error rate. The analysis is actually shown in Figure 7 in the original manuscript. This figure compared the amount of the data transmission under different similarity threshold as well as the fault error rate. It reveals that the incremental results can be compressed up to 90\% when the soft error rate is lower. This is mainly because that the neural network outputs change little under low soft error rate and there are a large number of zeros in the incremental results. In contrast, the incremental results get dense and are more difficult to compress when the soft error rate increases. 

\textbf{Q4: Section V-B. In critical layer protection, what is the difference or improvement (in theory) of the proposed heuristic from brute-force search? What’s the overhead for performing this search on different types of networks, particularly for the large and deep ones?} As the soft error induced computing errors propagate during the neural network processing, different protection of the layer combination can cause different model accuracy improvement. In this case, a brute-force search algorithm needs to evaluate $C(L,s)=\frac{L!}{s!\times (L-s)!}$ design options. The overhead can be extremely large given large neural network models. With the proposed heuristic selection algorithm, we need to evaluate $Sum(L,s)=\sum_{k=s+1}^{k=L}k=\frac{(L+s+1)\times (L-s)}{2}$ design options, which is much smaller. Take ResNet50 as an example, when $L=50$ and $s=5$, $C(L,s)=2118760$, $Sum(L,s)=240$. For the accuracy evaluation of each design option, suppose we conduct 1000 inferences with random soft error injection and it takes around 16 seconds for ResNet50. In this case, the total evaluation time of the brute-force search is more than 392 days, which is too long for practical employment. As a result, we only evaluate the proposed layer protection with the fully TMRed neural network models. We also improve the description in the Second Paragraph in Page 7.

\textbf{Q5: Section VI-A In addition to citing the Ares paper, the fault injection requires more explanation, particularly about when the errors are injected under the proposed design loop. E.g., does this paper use static injection or dynamic injection? Do the position of bit errors vary between different inferences, batches or epochs?} Although the soft errors in the neural network accelerator essentially are located in on-chip buffers and registers, they essentially affect the MAC operations in the neural network processing. To avoid lengthy RTL-based fault simulation, we have the random soft errors injected to the MAC operations including the input features, weights, and the output features in the neural network processing on CPU. Thereby, the fault injection is dynamic and the position of the bit errors vary across the different inferences, batches, and epochs. We also update the fault injection description in Section IV-A to clarify the fault injection issue.





==> figures/mycrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__

